Multiclass Classification, Information, Divergence, and Surrogate Risk

We provide a unifying view of statistical information measures, multi-way Bayesian hypothesis testing, loss functions for multi-class classification problems, and multi-distribution $f$-divergences, elaborating equivalence results between all of these objects, and extending existing results for binary outcome spaces to more general ones. We consider a generalization of $f$-divergences to multiple distributions, and we provide a constructive equivalence between divergences, statistical information (in the sense of DeGroot), and losses for multiclass classification. A major application of our results is in multi-class classification problems in which we must both infer a discriminant function $\gamma$---for making predictions on a label $Y$ from datum $X$---and a data representation (or, in the setting of a hypothesis testing problem, an experimental design), represented as a quantizer $\mathsf{q}$ from a family of possible quantizers $\mathsf{Q}$. In this setting, we characterize the equivalence between loss functions, meaning that optimizing either of two losses yields an optimal discriminant and quantizer $\mathsf{q}$, complementing and extending earlier results of Nguyen et. al. to the multiclass case. Our results provide a more substantial basis than standard classification calibration results for comparing different losses: we describe the convex losses that are consistent for jointly choosing a data representation and minimizing the (weighted) probability of error in multiclass classification problems.

==> proof-super-equivalence.tex <==
% -*- Mode: latex -*-

\section{Proof of Theorem \ref{theorem:equivalence-super}}
\label{sec:proof-equivalence-super}

We divide our proof into the three
cases~(\ref{item:no-domain})--(\ref{item:same-domain}). First, we show that
if any of the cases hold, then $f_1$ and $f_2$ are order equivalent.

It is clear that if $\dom f_1 = \dom f_2 = \varnothing$, then
Definition~\ref{def:order-equivalent} holds, as we have $\infty \le
\infty$.  In case~(\ref{item:unequal-domains}) of the theorem, 
both $f_1$ and $f_2$ are linear
linear on the convex cones $C_1 = \dom f_1$ and $C_2 = \dom f_2$.
If the matrices $A = [x_1 ~ \cdots ~ x_m]$ and $B = [y_1 ~ \cdots ~ y_m]
\in \R^{k \times m}_+$ satisfy
$x_i \in \dom f_1$ and $A \ones = B \ones$, then we have
$\frac{1}{m} A \ones = \frac{1}{m} B \ones \in \dom f_1$,
whence $y_i \in \dom f_1$ by the definition of the domain $\dom f_1
= \sum_{j \in I_{f_1}} \R_+ e_j$.
The same is true for $f_2$, so that we find we always have
\begin{equation*}
  \sum_{j=1}^m f_1(x_j) = \sum_{j=1}^m f_1(y_j)
  ~~ \mbox{and} ~~
  \sum_{j=1}^m f_2(x_j) = \sum_{j=1}^m f_2(y_j),
\end{equation*}
as $f_1$ and $f_2$ are linear or both sides are $+\infty$.  In
case~(\ref{item:same-domain}), we certainly have order equivalence of $f_1$
and $f_2$.

Now, suppose the converse, that is, that $f_1$ and $f_2$ are order
equivalent. We show that one of
cases~(\ref{item:no-domain})--(\ref{item:same-domain}) must hold.
For any two closed convex functions $f_1$  and $f_2$, we must
have one of $\dom f_1 = \dom f_2 = \varnothing$,
$\dom f_1 = \varnothing$ and $\dom f_2 \neq \varnothing$,
$\dom f_1 \neq \varnothing$ and $\dom f_2 = \varnothing$,
or $\dom f_1 \neq \varnothing$ and $\dom f_2 \neq \varnothing$. We
consider each in turn, identifying them with
cases~(\ref{item:no-domain}), (\ref{item:unequal-domains}),
and~(\ref{item:same-domain}).

\textbf{Case~(\ref{item:no-domain}).}
If $\domain{f_1} = \domain{f_2} = \varnothing$, we are done.

\textbf{Case~(\ref{item:same-domain}).}  We proved this in the main body of
the paper as Lemma~\ref{lemma:equivalence-subset2}.

\textbf{Case~(\ref{item:unequal-domains}).}
In the remaining case, we have $\domain{f_1} \neq \domain{f_2}$.
An important part of the proof is demonstrating
that the domains $\domain{f_i}$ have the structure
$\{x \in \R^k_+ \mid x_j = 0 ~ \mbox{for}~ j \in I\}$ for some index
set $I$. To that end, we present a definition and lemma that will
prove useful in the proofs of many of our subsequent results.
\begin{definition}
  \label{def:pierceable}
  We call a set $A \subset \R_{+}^k$ \emph{pierceable} if 
  for some $z \in A$ there exist $x, y \in \R_+^k \setminus A$ such
  that $\half(x + y) = z$.
\end{definition}
\noindent
This definition is intimately related to sets with the geometry
we desire in Case~(\ref{item:unequal-domains}).
\begin{lemma}
  \label{lemma:pierceable}
  Let $\Omega = A \cap \R_{+}^k \neq \varnothing$, where $A$ is
  affine and satisfies $A = \affine \Omega$. Then $\Omega$ is not
  pierceable if and only if there exists a set $I \subset [k]$
  such that $\Omega = \{x\in \R_{+}^k \mid x_j = 0 ~ \mbox{for}~ j \in I\}$.
\end{lemma}
\noindent
See Section~\ref{sec:proof-pierceable} for a proof of the lemma.

We divide our remaining discussion into the cases that one of $\domain{f_1}$
and $\domain{f_2}$ is the empty set $\varnothing$, or when $\domain{f_1}
\neq \varnothing$ and $\domain{f_2} \neq \varnothing$.

\paragraph{One of the domains of $f_1$ and $f_2$ is empty}

We consider the case that $\domain{f_1} = \varnothing$ and
$\domain{f_2} \neq \varnothing$.  Let $x \in \dom f_2$ with $x \in
\R^k_+$. Define the matrices $A = [x ~ x]$ and $B = [2x ~ \zeros] \in \R^{k
  \times 2}_+$. Then $A \ones = B \ones = 2x$, and using the equivalent
version~\eqref{eqn:equivalent-order-equivalence} of order equivalence, we
have $2 f_1(x) = f_1(2x) = +\infty$, so that $2 f_2(x) = f_2(2x) +
f_2(\zeros) < \infty$. In particular, $\zeros \in \dom f_2$.

%%   Moreover, for any
%%   rational number $(r/s) \in \Q_+$ with $r, s \in \N$, we may construct
%%   matrices
%%   \begin{equation*}
%%     A = \big[\underbrace{x ~ \cdots ~ x}_{r~{\rm times}}
%%       ~ \underbrace{0 ~ \cdots ~ 0}_{s-r~{\rm times}}\big]^T
%%     ~~ \mbox{and} ~~
%%     B = \frac{r}{s} \left[ x ~ \cdots ~ x\right]^T
%%     \in \R_+^{s \times k},
%%   \end{equation*}
%%   and $A^T\ones = B^T\ones = r x$, and $r f_2(x) + (s - r) f_2(0) = s
%%   f_2(\frac{r}{s} x)$ again using the equivalent
%%   version~\eqref{eqn:equivalent-order-equivalence} of order equivalence as
%%   $f_1 \equiv +\infty$. In particular, for any $x \in \dom f_2$, we have
%%   that $q x \in \dom f_2$ for any nonnegative rational $q \in \Q_+$; using
%%   the one-dimensional continuity of closed convex functions~\cite[Chapter
%%     I.3]{HiriartUrrutyLe93} we obtain that $\dom f_2$ contains the ray $\{tx
%%   \mid t \ge 0\}$ for all $x \in \dom f_2$, that is,
%%   $\dom f_2$ is a convex cone.

Now, we claim that if $x \in \dom f_2$, we have that for any set of
rational numbers $q \in \Q^m_+$ and $x_i \in \R_+^k$ satisfying $x =
\sum_{i = 1}^m q_i x_i$, then
\begin{equation}
  f_2(x) = \sum_{i=1}^m q_i f_2(x_i)
  + (1 - \ones^Tq) f_2(\zeros).
  \label{eqn:linear-funny-bunny}
\end{equation}
Indeed, let $q_i = r_i / s$ 
and if $s \ge r^T\ones$, define the matrices
\begin{equation*}
  A = [\underbrace{x ~ \cdots ~ x}_{s ~ {\rm times}}]
  ~~ \mbox{and} ~~
  B = [\underbrace{x_1 ~ \cdots ~ x_1}_{r_1 ~ {\rm times}}
    ~ \cdots ~ \underbrace{x_m ~ \cdots ~ x_m}_{r_m ~ {\rm times}}
    ~ \underbrace{\ones ~ \cdots ~ \ones}_{s - \ones^T r ~ {\rm times}}].
\end{equation*}
Then clearly $A \ones = s x = B \ones$, and $\infty = s f_1(x) =
\sum_{i=1}^m r_i f_1(x_i) + (s - \ones^T r) f_1(\zeros)$, so that by
inequality~\eqref{eqn:equivalent-order-equivalence} we have
\begin{equation*}
  s f_2(x) = \sum_{i=1}^m r_i f_2(x_i) + (s - \ones^Tr) f_2(\zeros).
\end{equation*}
On the other hand, if $s < r^T \ones$, define matrices
\begin{equation*}
  A = [\underbrace{x ~ \cdots ~ x}_{s ~ {\rm times}}
    ~ \underbrace{\zeros ~ \cdots ~ \zeros}_{\ones^Tr - s ~ {\rm times}}]
  ~~ \mbox{and} ~~
  B = [\underbrace{x_1 ~ \cdots ~ x_1}_{r_1 ~ {\rm times}}
    ~ \cdots ~ \underbrace{x_m ~ \cdots ~ x_m}_{r_m ~ {\rm times}}].
\end{equation*}
Then again we have $A \ones = sx = B \ones$, and again using order
equivalence (because $f_1 \equiv +\infty$) we obtain $s f_2(x) + (\ones^T
r - s) f_2(\zeros) = \sum_{i=1}^m r_i f_2(x_i)$.  In either case, we find that
equation~\eqref{eqn:linear-funny-bunny} holds.  In particular, $f_2(x_i) <
\infty$ whenever $x \in \dom f_2$ and $x = \sum_{i=1}^m q_i x_i$ for some
$q_i \in \Q_+$.  Thus, taking $x_1 = tx$ and $q = 1/t$ as $t \to \infty$
in $\Q$, we have that $f_2(tx) = t f_2(x) + (1 - t) f_2(\zeros)$ and $t x \in
\dom f_2$.  Using the one-dimensional continuity of closed convex
functions~\cite[Chapter I.3]{HiriartUrrutyLe93} we obtain that $\dom f_2$
contains the ray $\{tx \mid t \ge 0\}$ for all $x \in \dom f_2$, that is,
$\dom f_2$ is a convex cone. Moreover, $f_2$ is affine along any
ray $\{tx \mid t \ge 0\}$.

If we take $q_i = 1$ and $x = \sum_{j=1}^k x_j e_j$ (where the $e_j \in
\R^k$ are standard basis vectors) then
for some $b, c \in \R^k$, expression~\eqref{eqn:linear-funny-bunny} becomes
\begin{equation*}
  f_2(x) = \sum_{j=1}^k f_2(x_j e_j) + (1 - k) f_2(\zeros)
  = \sum_{j=1}^k (b_j x_j + c_j) + (1 - k) f_2(\zeros),
\end{equation*}
where in the second equality we have used that $f_2$ is affine along any
ray. In particular, if $x_j > 0$ for a vector $x \in \dom f_2$, then
$f_2(e_j) < \infty$, and we have proved case~(\ref{item:unequal-domains})
when $\domain{f_1} = \varnothing$ and $\domain{f_2} \neq \varnothing$.  The
case that $\domain{f_2} = \varnothing$ and $\domain{f_1} \neq \varnothing$
is parallel.

\paragraph{Both domains of $f_1$ and $f_2$ are non-empty}

It remains to prove case~(\ref{item:unequal-domains}) of
Theorem~\ref{theorem:equivalence-super} when both $\domain{f_1} \neq
\varnothing$ and $\domain{f_2} \neq \varnothing$.  We divide our discussion
into the cases that $\dom f_1 \cap \dom f_2 \neq \varnothing$ and $\dom f_1
\cap \dom f_2 = \varnothing$.

\paragraph{The domains of $f_1$ and $f_2$ have non-empty intersection}

First, we consider the case that $\domain{f_1} \cap \domain{f_2} \neq
\varnothing$.  Let $H = \affine{\{\domain{f_1} \cap \domain{f_2}\}}$
be the affine hull of $\dom f_1 \cap \dom f_2$ and $H_+ = H \cap \R_+^k$
be its intersection with the positive orthant. We have the following
lemma.
\begin{lemma}
  \label{lemma:domains-same-on-hull}
  Under the conditions of the preceding paragraph,
  we have
  \begin{equation}
    \label{eqn:domains-same-on-hull}
    \dom f_1 \cap H = \dom f_2 \cap H,
  \end{equation}
  and $\dom f_1 \cap \dom f_2 \cap H_+ \neq \varnothing$.
\end{lemma}
\noindent
That is, $f_1$ and $f_2$ have the same domain on the affine hull of the
intersection $\domain{f_1} \cap \domain{f_2}$. (See
Section~\ref{sec:proof-domains-same-on-hull} for a proof of
Lemma~\ref{lemma:domains-same-on-hull}.)

Lemma~\ref{lemma:equivalence-subset2} applies on $\dom f_1 \cap \dom
f_2$---that is, we have $f_1(t) = a f_2(t) + b^T t + c$ for $t \in \dom f_1
\cap H = \dom f_2 \cap H$---so we need only consider the behavior of the
$f_i$ off of $H$. That is, if $\dom f_1 \setminus H = \dom f_2 \setminus H =
\varnothing$, then Lemma~\ref{lemma:domains-same-on-hull} implies that $\dom
f_1 = \dom f_2$, we have $f_1 = f_2 = \infty$ on the set $H^c$, and
Lemma~\ref{lemma:equivalence-subset2} implies that $f_1(t) = a f_2(t) + b^T t
+ c$ for all $t$, where $a > 0$ and $b \in \R^k, c \in \R$. Thus we have
completed the proof of Case~(\ref{item:unequal-domains}) when $H =
\affine{\dom f_1 \cap \dom f_2} \supset \dom f_1$ and $H \supset \dom f_2$.

Now, suppose that $\dom f_1 \setminus H \neq
\varnothing$, and define $\Omega_1 = \domain{f_1} \setminus H$. Note that
$f_2(x) = +\infty$ for all $x \in \Omega_1$ by definition of $H$.
We have
\begin{claim}
  \label{claim:convex-subset}
  The set $\Omega_1 = \domain{f_1} \setminus H$ is convex.
\end{claim}
\begin{proof}
  Claim~\ref{claim:convex-subset} is a consequence of the order equivalence
  of $f_1$ and $f_2$, which we prove by showing that if $x_1, x_2 \in
  \Omega_1$ then $x_3 = \half(x_1 + x_2) \not \in H$ (while $x_3 \in \dom
  f_1$ so that $x_3 \in \Omega_1 = \dom f_1 \setminus H$).
  By definition of $H$, we have $f_2(t) = +\infty$ for all $t \in \Omega_1$.
  For the sake of contradiction, suppose that $x_3 \in H$ while $x_1 \neq
  x_2$ (when $x_1 = x_2$ it is clear that $x_3 \not \in H$).  Then by
  convexity of $\domain{f_1}$, we have $x_3 \in H \cap
  \domain{f_1}$. Lemma~\ref{lemma:domains-same-on-hull} implies that $H \cap
  \dom f_1 = H \cap \dom f_2$, and thus in this case $f_1(x_3) < \infty$ and
  $f_2(x_3) < \infty$. As $x_1, x_2 \not \in \dom f_2$, we have $\half
  (f_2(x_1) + f_2(x_2)) > f_2(x_3)$, and order equivalence
  (Def.~\ref{def:order-equivalent}) implies that
  \begin{equation*}
    \half (f_1(x_1) + f_1(x_2)) > f_1(x_3).
  \end{equation*}
  By construction of $H$ as an affine space and the assumption that $x_3 \in
  H$ while $x_1, x_2 \not \in H$, we have for all $\epsilon \in (0, 1)$ that
  \begin{equation*}
    x_\epsilon \defeq
    x_3 + \frac{\epsilon}{2}(x_1 - x_2)
    = \frac{1 + \epsilon}{2} x_1 + \frac{1 - \epsilon}{2} x_2 \not \in H.
  \end{equation*}
  In particular, $x_\epsilon \in \Omega_1$ as $x_\epsilon \in \dom f_1$,
  while $x_\epsilon \not \in \dom f_2$.
  By noting that
  \begin{equation*}
    \frac{1+\epsilon}{2}f_2(x_1) +
    \frac{1-\epsilon}{2}f_2(x_2) = +\infty = f_2(x_{\epsilon}),
  \end{equation*}
  we have, by order equivalence, that $f_1(x_{\epsilon}) =
  \frac{1+\epsilon}{2}f_1(x_1) + \frac{1-\epsilon}{2}f_1(x_2)$. Using
  the continuity of one-dimensional closed convex functions,
  taking $\epsilon \to 0$ yields $f_1(x_3) = \half (f_1(x_1) + f_2(x_2))$,
  a contradiction to our earlier strict inequality. Thus
  $\Omega_1 = \dom f_1 \setminus H$ is convex.
\end{proof}

It remains to show that $f_1$ is a linear function on $\Omega_1$. Let us
assume that $\dim(\Omega_1) = l \geq 1$. As $\Omega_1$ is convex, we may use
our earlier results (Lemma~\ref{lemma:sub-simplices}) to see that $f_1$ is
linear on $\Omega_1$ if and only if for all sets $E \subset \Omega_1$ of the
form $E = \conv\{x_0, \ldots, x_l\}$ with the $x_i$ affinely independent
(Def.~\ref{def:affine-independent}), $f_1$ is linear in $E$.
Take such a set $E$. Then for all $x \in E$, we have $f_2(x) = +\infty$, and
so for $\alpha \in \Q^{l+1}_+$ with $\ones^T \alpha = 1$,
\begin{equation*}
  f_2 \left(\sum_{i=0}^l \alpha_i x_i \right)
  = \sum_{i=0}^{l}  \alpha_i f_2(x_i) = +\infty,
  ~~~ \mbox{so} ~~~
  f_1 \left(\sum_{i=0}^l \alpha_i x_i \right)
  = \sum_{i=0}^{l}  \alpha_i f_1(x_i)
\end{equation*}
by Eq.~\eqref{eqn:order-equivalent-equality} and order equivalence.
That is, $f_1$ is linear on $E_\Q \defeq \{x = \sum_{i=0}^l \alpha_i x_i
\mid \alpha \in \Q_+^k, \ones^T \alpha = 1\}$. As $E_\Q$ is dense in $E =
\conv\{x_0, x_1, \ldots, x_l\}$, Lemma~\ref{lemma:equal-functions} implies
that $f_1$ is linear on $E$, and Lemma~\ref{lemma:sub-simplices} implies that
\begin{equation*}
  f_1(t) = b_1^T t + c_1 ~~ \mbox{for}~ t \in \Omega_1 = \dom f_1 \setminus H.
\end{equation*}

We now show that $f_1$ is linear on $\domain{f_1} \supset \Omega_1$.
As $\Omega_1 \neq \varnothing$, one may choose a point $x \in
\Omega_1$.  For all $y \in H \cap \domain{f_1}$, the segment $S_{xy} =
\{\lambda x + (1 - \lambda) y \mid \lambda \in [0, 1]\} \subset \dom f_1$,
and because $H$ is an affine space, $S_{xy} \setminus \{y\} \subset
\Omega_1$.  As $S_{xy}$ is one-dimensional and $f_1$ is closed convex, it is
continuous on $S_{xy}$ (e.g.~\cite[Chapter I]{HiriartUrrutyLe93}), and thus
we have $f_1(t) = b_1^Tt + c_1$ for all $t \in S_{xy}$, including $y$.  As
$y \in H\cap \domain{f_1}$ is arbitrary, the linearity of $f_1$ on
$\Omega_1$ extends to all of $H \cap \dom f_1$, and thus $f_1$ is linear on
its domain.
%
By a symmetric argument to that above, we obtain that
$f_2$ is linear on the convex set $\Omega_2 = \dom f_2 \setminus H$,
and we find that $f_2$ is similarly linear on $\dom f_2$.

Finally, we state a lemma (whose technical proof we defer
to Section~\ref{sec:proof-characterization-linear}) showing
that the domains of $f_1$ and $f_2$ take the form asserted in
Case~(\ref{item:unequal-domains}).
\begin{lemma}
  \label{lemma:characterization-linear}
  Let $f_1 : \R^k_+ \to \extendedR$ and $f_2 : \R^k_+ \to \extendedR$ be order
  equivalent (Def.~\ref{def:order-equivalent}) and linear on their domains,
  which we assume satisfy $\domain{f_1} \neq \varnothing$, $\domain{f_2} \neq
  \varnothing$ and $\domain{f_1} \cap \domain{f_2} \neq \varnothing$.  In
  addition, let $H = \affine\{\domain{f_1} \cap \domain{f_2}\}$ and assume
  that $H \cap \domain{f_1} = H \cap \domain{f_2}$ and $\domain{f_1}
  \backslash H$ is convex and non-empty.  Then there exist index sets
  $I_{f_1}, I_{f_2} \subset [k]$ such that
  \begin{equation*}
    \domain{f_i} = \{x\in \R_+^k \mid x_j = 0 \text{ for } j\in I_{f_i}\}.
  \end{equation*}
\end{lemma}
\noindent
We have shown that the conditions of
Lemma~\ref{lemma:characterization-linear} are satisfied, so
there exist sets $I_1, I_2 \subset [k]$ such that
$\domain{f_1} = \{x \in \R_+^k \mid x_j = 0 \text{ for } j \in I_1\}$ and
$\domain{f_2} = \{x \in \R_+^k \mid x_j = 0 \text{ for } j \in I_2\}$.


\paragraph{The domains of $f_1$ and $f_2$ have empty intersection}

Now we return to the case that $\domain{f_1} \cap \domain{f_2} =
\varnothing$. Identical reasoning to our derivation that $f_1$ is linear on
$\Omega_1 = \domain{f_1} \setminus \affine \{\dom f_1 \cap \dom f_2\}$ in
the case that $\domain{f_1} \cap \domain{f_2} \neq \varnothing$ shows that
$f_1$ must be linear on the complement of $\dom f_2$.  Similarly, $f_2$ must
be linear on the complement of $\dom f_1$.  The next lemma implies that
$\dom f_1 \cap \dom f_2 \neq \varnothing$, which means that our assumption
that $\domain{f_1} \cap \domain{f_2} = \varnothing$ cannot occur, completing
the proof of case~(\ref{item:unequal-domains}) of
Theorem~\ref{theorem:equivalence-super}. See
Sec.~\ref{sec:proof-nonempty-intersection} for a proof of
Lemma~\ref{lemma:nonempty-intersection}.
\begin{lemma}
  \label{lemma:nonempty-intersection}
  Suppose two order equivalent functions $f_1 : \R^k_+ \to \extendedR$ and
  $f_2 : \R^k_+ \to \extendedR$ are linear in their domains with
  $\domain{f_1} \neq \varnothing$ and $\domain{f_2} \neq \varnothing$. Then
  $\domain{f_1} \cap \domain{f_2} \neq \varnothing$.
\end{lemma}

\subsection{Proof of Lemma~\ref{lemma:pierceable}}
\label{sec:proof-pierceable}

Assume that $\Omega$ is not pierceable.  Let $l = \dim{A}\geq 0$ and
$\lzero{x}$ be the $\ell_0$-norm (number of non-zeros) of the vector
$x$. Define $m = \max \{\lzero{x} \mid x \in \Omega\}$; we show that if $m
> l$, then $\Omega$ must be pierceable.  Indeed, assume that $m > l$ and
take $z \in \Omega$ with $m$ non-zero components. Without loss, we assume
that $z = (z_1, \ldots, z_m, 0, \ldots, 0)$. For $\epsilon \in \R$ and $i
= 1, \ldots, m$, consider the pairs $x_i^\epsilon = z + \epsilon e_i$ and
$y_i^\epsilon = z - \epsilon e_i$, where $e_i$ are the standard basis
vectors. As $A$ has dimension $l < m$, there must be some index $i^*$ such
that both $x_{i^*}^\epsilon \not \in A$ and $y_{i^*}^\epsilon \not \in A$
for all $\epsilon \in (0, z_{\min})$, where $z_{\min} = \min\{z_i \mid z_i
\neq 0\}$.  In particular, $x_{i^*}^\epsilon, y_{i^*}^\epsilon \in \R_+^k
\setminus A$ and $z = \half(x_{i^*}^\epsilon + y_{i^*}^\epsilon)$, so that
$\Omega$ is pierceable. That is, if $\Omega$ is not pierceable, we must
have that
\begin{equation*}
  m = \max\{\lzero{x} \mid x \in \Omega\}
  \le \dim A = l.
\end{equation*}

Thus for any affine set $A$, if $\Omega$ is not pierceable, we have for
$m = \max\{\lzero{x} \mid x \in \Omega\} \le \dim A$ that
\begin{equation*}
  \Omega \subset \bigcup_{I \subset [k],
    |I| = m} \left\{x \in \R^k_+ \mid x_j = 0 ~ \mbox{for}~
  j \not \in I \right\}.
\end{equation*}
This is a union of different subspaces (restricted to the positive
orthant); by the convexity of $\Omega$, there must be some $I \subset [k]$
with $|I| = m$ such that $\Omega \subset \{x \in \R_+^k \mid x_j = 0 ~
\mbox{for} ~ j \not\in I\}$.  (We have $I = [k]$ if $\dim A = k$.)  We
show that $\Omega = \{x \in \R^k_+ \mid x_j = 0 ~ \mbox{for}~ j \not\in
I\}$.  Without loss of generality, assume that $I = \{m + 1, \ldots, k\}$.
Then there exists a vector $x \in \Omega$ such that
$x = (x_1, \ldots, x_m, 0, \ldots, 0)$, with $x_j \neq 0$ for $j \le m$.
Because $l = \dim A \ge m$ and $A$ is affine, we may represent
$A$ as $A = \{Fv + g \mid v \in \R^l\}$ for a matrix $F \in \R^{k \times l}$.
It then must be the case that
$z \in A$ implies that $z_j = 0$ for all $j \in I$ by continuity
of $v \mapsto Fv + g$, and moreover, as $m \le l$, we then must have
$(x_1, \ldots, x_m, 0, \ldots, 0) \in A$ for all $x_1, \ldots, x_m$. That
is, $\Omega = \{x \in \R_+^k \mid x_j = 0 ~ \mbox{for}~ j \not\in I\}$.

Conversely, suppose there exists a set $I \subset [k]$ such that $\Omega =
\{x \in \R^k_+ \mid x_j = 0 ~ \mbox{for}~ j \in I\}$.  Then any $x, y \in
\R^k_+$ such that $\half (x + y) \in \Omega$ must have $x_j = y_j = 0$ for
all $j \in I$. But then $x, y \in \Omega$, which contradicts
Definition~\ref{def:pierceable}.  

\subsection{Proof of Lemma~\ref{lemma:domains-same-on-hull}}
\label{sec:proof-domains-same-on-hull}

We consider the common domain $\Omega = \domain{f_1} \cap \domain{f_2}$
and its intersection with $H_+$. That $\dom f_1 \cap \dom f_2 \cap H_+
\neq \varnothing$ is an immediate consequence of our assumption that $H
= \affine{\dom f_1 \cap \dom f_2}$ and $\dom f_i \subset \R^k_+$.
In addition, we note that if $\dom f_1 \cap \dom f_2$ is a single
point, then the lemma immediately follows, so we may assume
that $\dom f_1 \cap \dom f_2$ contains more than a single point.

Let $A_1 = \relint \{\domain{f_1}\cap
H_+\}$ and $A_2 = \relint \{\domain{f_2}\cap H_+\}$, which are non-empty
by construction of $H$, and additionally satisfy $A_1 \cap A_2 \neq
\varnothing$ because $\dom f_1 \cap \dom f_2$ contains more than a single
point. We claim that
\begin{equation}
  \label{eqn:interiors-same-on-affine}
  \relint \{\dom f_1 \cap H_+\} = A_1 = A_2
  = \relint \{\dom f_2 \cap H_+\}.
\end{equation}
Deferring temporarily the proof of the
claim~\eqref{eqn:interiors-same-on-affine}, we show how it yields
equation~\eqref{eqn:domains-same-on-hull}.  Indeed, $H_+$ and $\dom f_i$ are
both closed and convex, whence $\dom f_i \cap H_+$ is closed convex, so that
$\cl A_i = \dom f_i \cap H_+$, while if $A_1 = A_2$ are convex then $\cl A_1
= \cl A_2$ (see, e.g~\cite[Proposition III.2.1.8]{HiriartUrrutyLe93}).
Thus $\dom f_1 \cap H = \dom f_1 \cap H_+ = \dom f_2 \cap H_+
= \dom f_2 \cap H$.

%% By
%% Lemma~\ref{lemma:equivalence-subset}, there exist
%% $a > 0, b \in \R^k, c \in \R$ such that
%% $f_1(t) = a f_2(t) + b^T t + c$ for all $t \in A = A_1 = A_2$, and
%% by Lemma~\ref{lemma:equal-functions}, this extends to
%% $\cl A$, so that $\dom f_1 \cap H_+ = \dom f_2 \cap H_+$, which
%% yields expression~\eqref{eqn:domains-same-on-hull}.

Now, we prove the claim~\eqref{eqn:interiors-same-on-affine}.  By
Lemma~\ref{lemma:equivalence-subset}, there exist $a > 0, b\in \R^k, c \in
\R$ such that
\begin{equation}
  \label{eqn:good-ordering-in-a1-cap-a2}
  f_1(t) = a f_2(t) + b^T t + c
  ~~ \mbox{for all} ~ t \in A_1 \cap A_2.
\end{equation}
Suppose for the sake of contradiction that $A_1 \neq A_2$. 
Without loss of generality, we may assume that $A_1 \not \supset A_2$.
Let $A = A_1 \cap A_2$, so
\begin{equation*}
  \relbd{A} =\relbd{\{A_1 \cap A_2\}} = 
  (\relbd{A_1} \cap \relbd{A})
  \cup (\relbd{A_2} \cap \relbd{A}).
\end{equation*}
We first choose two distinct points $x, y$ such that
\begin{equation}
  x \in \relbd{A_2} \cap \relint A_1
  ~~ \mbox{and} ~~
  y \in \relint A.
  \label{eqn:distinct-x-y-choice}
\end{equation}
To see that we may make such a choice for $x$, let
$B_1 = \relbd{A_1} \cap \relbd{A} $ and $B_2 = \relbd{A_2}
\cap \relbd{A}$ be the boundary parts of $A$ corresponding to $A_1$ and
$A_2$; we claim
\begin{claim}
  \label{claim:bd}
  With the above assumptions, $B_2 \setminus B_1 \neq \varnothing$.
\end{claim}
\noindent
We defer the proof of the claim to the end of this section
and continue with the proof of the
equality~\eqref{eqn:interiors-same-on-affine}.  Claim~\ref{claim:bd} allows
us to take a point $x \in B_2 \backslash B_1$. Then we have that $x\in
\relbd{A_2} \cap \relbd{A} $ and $x \not\in \relbd{A_1}$. Additionally, as
$x$ is an accumulation point of $A \cap H_+$ satisfying $x \not \in
\relbd{A_1}$, it must be the case that $x \in \relint A_1$ (this is relative
to $H_+$ by construction of the sets $A_i$).  In particular, $f_1(x) <+
\infty$ and we have $x$ and $y$ as desired~\eqref{eqn:distinct-x-y-choice}.

We show that $f_2(x)$ is finite.
Define the sequence $x_i = \frac{1}{i + 1} (i x + y)$ for $i = 1, 2,
\ldots$. As $x \in B_2 \subset \relbd{A}$, we have $x_i \in \relint A$ for
all $i$ by Lemma~\ref{lemma:interior-line-segments}, while $x_i \to x$ as $i
\to \infty$.  Therefore, $f_1(x_i) = af_2 (x_i) + b^T x_i + c$ by
expression~\eqref{eqn:good-ordering-in-a1-cap-a2}, and $f_1(x_i) <+\infty$
and $f_2(x_i) <+ \infty$ for all $i$.  Since closed convex functions are
continuous in one dimension~\cite[Chapter I.3]{HiriartUrrutyLe93}, by
restricting $f_1$ and $f_2$ to the line $\{\lambda x + (1 - \lambda) y \mid
\lambda \in [0, 1]\}$, we take limits to obtain that
\begin{equation*}
  f_2(x) =
  \lim_{i \to \infty} a^{-1}\left(f_1(x_i) - b^T x_i - c\right)
  = a^{-1} (f_1(x) - b^T x - c) < \infty.
\end{equation*}

As $x, y \in \relint A_1$, there must exist
some $\delta \in (0, 1)$ such that for $\epsilon \in (0, \delta)$,
we have $(1 + \epsilon) x - \epsilon y \in A_1$. On the other
hand, we know that $x$ is on the relative boundary of $A_2$ with
$y \in \relint A_2$,
and thus $(1 + \epsilon) x - \epsilon y \not \in A_2$, that is,
$f_2((1 + \epsilon) x - \epsilon y) = \infty$ for all such $\epsilon$.
Now we use the order equivalence (Def.~\ref{def:order-equivalent})
of $f_1$ and $f_2$. We have
\begin{equation}
  \label{eqn:f2-big-A-boundary}
  \infty = f_2\left(\left(1 + \frac{\epsilon}{2}\right) x
  - \frac{\epsilon}{2} y\right) +
  f_2\left(\left(1 - \frac{\epsilon}{2}\right) x
  + \frac{\epsilon}{2} y \right)
  > 2 f_2(x) \neq \infty,
\end{equation}
while on the other hand, for any $\epsilon' \in (0, \epsilon)$ we have
\begin{equation*}
  f_2\left(\left(1 + \frac{\epsilon}{2}\right) x
  - \frac{\epsilon}{2} y\right) +
  f_2\left(\left(1 - \frac{\epsilon'}{2}\right) x
  + \frac{\epsilon'}{2} y \right)
  = +\infty =
  2 f_2\left(\left(1 + \frac{\epsilon - \epsilon'}{4}\right) x
  - \frac{\epsilon - \epsilon'}{4} y\right).
\end{equation*}
Thus, by order equivalence, we must have
\begin{equation*}
  f_1\left(\left(1 + \frac{\epsilon}{2}\right) x
  - \frac{\epsilon}{2} y\right) +
  f_1\left(\left(1 - \frac{\epsilon'}{2}\right) x
  + \frac{\epsilon'}{2} y \right)
  = 2 f_1\left(\left(1 + \frac{\epsilon - \epsilon'}{4}\right) x
  - \frac{\epsilon - \epsilon'}{4} y\right)
\end{equation*}
whenever $\half \delta > \epsilon > \epsilon' > 0$. Using the
one-dimensional continuity of closed convex functions and taking
$\epsilon' \uparrow \epsilon$, the previous display implies that
\begin{equation*}
  f_1\left(\left(1 + \frac{\epsilon}{2}\right) x
  - \frac{\epsilon}{2} y\right) +
  f_1\left(\left(1 - \frac{\epsilon}{2}\right) x
  + \frac{\epsilon}{2} y \right)
  = 2 f_1(x),
\end{equation*}
which contradicts the order equivalence of $f_1$ and $f_2$ and
inequality~\eqref{eqn:f2-big-A-boundary}. This in turn contradicts the
existence~\eqref{eqn:distinct-x-y-choice} of our points $x, y$, which were
predicated on $A_1 \neq A_2$, so that
equation~\eqref{eqn:interiors-same-on-affine} holds.

%% \begin{lemma}
%%   Let $A_1, A_2$ be convex sets, and assume that $A = A_1 \cap A_2 \neq
%%   \varnothing$ and $\affine{A} = \affine{A_1} = \affine{A_2}$.  In addition,
%%   assume that $A_1$ and $A_2$ are relatively open.  If $A_2 \not \supset
%%   A_1$ and we set $B_1 = \relbd A_1 \cap \relbd A$ and $B_2 = \relbd A_2
%%   \cap \relbd A$, then $B_2 \setminus B_1 \neq \varnothing$.
%% \end{lemma}
Finally, we return to prove the Claim~\ref{claim:bd}.

\begin{proof-of-claim}[\ref{claim:bd}]
  Because their affine hulls are identical, we may without loss of
  generality assume that $A_1$ and $A_2$ are open sets. We must have
  $A_1 \setminus \cl A_2 \neq \varnothing$, as otherwise we would have $A_1
  \subset \interior{\cl A_2} = A_2$ as $A_1$ is open.
  We now construct a point in $B_2$ that is not in $B_1$.
  Let $x \in A_1 \setminus \cl A_2$ and $y \in A = A_1 \cap A_2$;
  then as $A_1 \setminus \cl A_2$ and $A$ are open, we must have
  \begin{equation*}
    t^* = \inf\left\{t \in [0, 1] \mid tx + (1 - t) y \not \in A_2 \right\}
    > 0,
  \end{equation*}
  as $A_2^c$ is closed.

  By the convexity of $A_2$, for all $t \in \openleft{t^*}{1}$ we have $tx +
  (1 - t)y \not \in A_2$ and for $t \in \openright{0}{t^*}$ we have $tx + (1
  - t) y \in A_2$. Moreover, for all $t \in [0, 1]$, we have $tx + (1 - t)y
  \in A_1$ by the convexity of $A_1$ and assumption that $x, y \in A$. In
  particular, we find that $t^* x + (1 - t^*) y \in \bd A_2 \cap \bd A =
  B_2$, while as $A_1$ is open we must have $tx + (1 - t) y \not \in \bd A_1
  \subset B_1$.  That is, we have $t^* x + (1 - t^*) y \in B_2$ while $t^* x
  + (1 - t^*) y \not \in B_1$, giving the claim
\end{proof-of-claim}

\subsection{Proof of Lemma~\ref{lemma:characterization-linear}}
\label{sec:proof-characterization-linear}

We know that $\dom f_1$ and $\dom f_2$ are closed convex sets, as each of
the $f_i$ are linear, so that as $\epi f_i$ are closed we must have $\dom
f_i$ closed.  For the remainder of the proof, let $\Omega_1 = \dom f_1
\setminus H$ and $\Omega_2 = \dom f_2 \setminus H$, so that $\Omega_1$ is
convex and $\Omega_1 \cap \Omega_2 = \varnothing$.  In addition, let $L =
\dom f_1 \cap H = \dom f_2 \cap H$ and
\begin{equation*}
  H_+ = (\affine{L}) \cap \R_+^k.
\end{equation*}

First, we show that we must have $L = H_+$, so that $L = \dom f_1 \cap H$ is
an affine space restricted to the positive orthant; subsequently we show
that $L$ is not pierceable (Def.~\ref{def:pierceable}), so that
Lemma~\ref{lemma:pierceable} yields the desired domains.  Suppose to the
contrary that $L \neq H_+$, so that one may choose a point $x \in H_+
\setminus L$. By assumption, $\Omega_1$ is convex, and thus we may also
choose $y \in \relint \Omega_1$; as $\dom f_1$ is closed we must have $x
\not \in \dom f_1$ and similarly $x \not \in \cl \Omega_1$.  Therefore,
standard convex analysis (cf.\ Lemma~\ref{lemma:interior-line-segments})
guarantees the existence of $t^* \in (0, 1)$ such that $z = t^*x + (1 -
t^*)y \in \relbd \Omega_1$. Now, as $t^* \in (0, 1)$ and $y \not \in H_+$,
we must have $z \not \in H_+$ and so $z \in \Omega_1$ (as we must have
either $z \in H_+$ or $z \in \Omega_1$).  This implies that $z \not \in \dom
f_2$, whence $f_2(z) = +\infty$. As $z \not \in \dom f_2$ (which is closed),
there must exist some $\epsilon > 0$ such that
\begin{equation*}
  z_\epsilon = z + \epsilon(x - z) \not \in \dom f_2
  ~~ \mbox{and} ~~
  z_{-\epsilon} = z - \epsilon(x - z) \not \in \dom f_2.
\end{equation*}
Noting that we have $f_2(z_{\epsilon}) + f_2(z_{-\epsilon}) = +\infty =
2f_2(z)$ and $f_1(z_{\epsilon}) + f_1(z_{-\epsilon}) = + \infty > 2f_1(z)$
yields a contradiction to the order equivalence of $f_1$ and $f_2$. Thus,
as claimed, we
must have
\begin{equation*}
  \dom f_1 \cap H = \dom f_2 \cap H = L = H_+ = (\affine{L}) \cap \R^k_+.
\end{equation*}

We now show that if we define $H_1 = \affine{\dom f_1} \cap \R_+^k$,
we have
\begin{equation}
  \label{eqn:linears-have-affine-domain}
  \dom f_1 = H_1
  = \affine \dom f_1 \cap \R_+^k.
\end{equation}
For the sake of contradiction, assume that $H_1 \neq \dom f_1$,
so that $H_1 \supsetneq \dom f_1$. Let $x \in H_1 \setminus \dom f_1$
and $y \in \relint \dom f_1$. Then, as $\dom f_1$ is closed,
as in the preceding paragraph there exists some $t^* \in (0, 1)$
such that $z = t^* x + (1 - t^*) y \in \relbd \dom f_1$.
We make the following intermediate claim:
if $x \not \in \dom f_1$ and $y \in \dom f_1$, then
\begin{equation}
  \label{eqn:hyperplaned-f1-domain-nope}
  t y + (1 - t) x \not \in H \cap \dom f_1
  ~~ \mbox{for}~ t \in (0, 1).
\end{equation}
Deferring the proof of the containment
relation~\eqref{eqn:hyperplaned-f1-domain-nope}, note that it implies we
must have $z \not \in H$, as we have $z \in \dom f_1$.  Thus $z \in
\Omega_1$, so that $z \not \in \dom f_2$, and by the fact that $\dom f_2$ is
closed, there must exist $\epsilon > 0$ such that $z_\epsilon = (1 +
\epsilon) z - \epsilon x \not \in \dom f_2$, and similarly $z_{-\epsilon} =
(1 - \epsilon) z + \epsilon x \not \in \dom f_2$.  Additionally,
$z_{-\epsilon} \not \in \dom f_1$ because $x \not \in \dom f_1$ and $z \in
\relbd \dom f_1$ (see Lemma~\ref{lemma:interior-line-segments}). Thus we
have
\begin{equation*}
  f_2(z_{-\epsilon}) + f_2(z_\epsilon) = 2 f_2(z) = +\infty,
\end{equation*}
which contradicts the fact that $f_1$ and $f_2$ are order equivalent and $2
f_1(z) < \infty = f_1(z_{-\epsilon}) + f_1(z_\epsilon)$.  Thus, accepting
temporarily the claim~\eqref{eqn:hyperplaned-f1-domain-nope}, we see that
$\dom f_1 = H_1$ as claimed~\eqref{eqn:linears-have-affine-domain}.

We return now to the containment
claim~\eqref{eqn:hyperplaned-f1-domain-nope}. Fix $y \in \domain{f_1}$ and
$x \not \in \dom f_1$, and assume for the sake of contradiction that there
exists $t^* \in (0, 1)$ such that $z = t^* y + (1-t^*)x \in H \cap
\domain{f_1}$. Now, since $x \not\in \domain{f_1}$, we must have $x \not \in
H_+ = \dom f_1 \cap H$.  By convexity of $\dom f_1$, we must also have for
$t \in \Q_+$ such that $t^* < t < 1$, if we define $u = t y + (1 - t) x$
then $u \in \dom f_1$.  Of course, as $u, y, x, z$ are collinear and $z \in
H_+ = \dom f_1 \cap H$ and $x \not \in H_+$, we must have $u \not \in H_+$,
whence $u \in \Omega_1 = \dom f_1 \setminus H$ and $u \not \in \dom
f_2$. Noting that
\begin{equation*}
  t f_1(x) + (1 - t) f_1(y) = \infty > f_1(u)
  ~~ \mbox{and} ~~
  t f_2(x) + (1 - t) f_2(y) = \infty = f_2(u),
\end{equation*}
we have a contradiction to the order equivalence of
$f_1$ and $f_2$ by Lemma~\ref{lemma:order-equivalence-rationals}.
That is, the claim~\eqref{eqn:hyperplaned-f1-domain-nope} must hold.

%%   Then, denote $H_1 = \affine{\domain{f_1}} \cap \R_{+}^k$ and $H_2 =
%%   \affine{\domain{f_2}} \cap \R_{+}^k$. We are going to show that
%%   $\domain{f_1} = H_1$. Suppose on the contrary, then one can pick up $x^* \in
%%   H_1 \backslash \domain{f_1}$ and $y \in \relint{\domain{f_1}}$.  Since
%%   $\domain{f_1}$ is closed, we have $x^*$ belong to the relative exterior of
%%   $\domain{f_1}$. Hence, standard convex analysis shows that there exists some
%%   $t^* \in (0, 1)$ such that $z^* = t^* x^* + (1-t^*) y^*$ belongs to the
%%   $\relbd {\domain{f_1}}$. Now, notice that by $z^*$ can not be some point in
%%   $H$ and hence $z^* \in J_1$, which means that $z^* \not\in
%%   \domain{f_2}$. Hence, there exist some $\epsilon >0$ such that $
%%   z^*_{\epsilon} = (1+\epsilon) z^* - \epsilon x^* \not\in \domain{f_2}$.  Now
%%   consider $z^* _{-\epsilon} = (1-\epsilon) z^* + \epsilon x^*$.  Then by
%%   convexity of $\domain{f_1}$ and Lemma \ref{lemma:interior-line-segments}, we
%%   have $z^*_{-\epsilon}\not\in \domain{f_1}$. Now, notice that since
%%   $\domain{f_1} \cap \domain{f_2} = \varnothing$, we have
%%   $f_2(z^*_{-\epsilon}) + f_2(z^*_{\epsilon}) = 2f_2(z^*) = +\infty$.  Hence,
%%   by order equivalence, we should have $f_1(z^*_{-\epsilon}) +
%%   f_1(z^*_{\epsilon}) = 2 f_1(z^*)$, which can not be true since
%%   $f_1(z^*_{-\epsilon}) + f_1(z^*_{\epsilon}) = +\infty$, while $f_1(z^*)$ is
%%   finite. Contradiction! Hence, we have $H_1 = \domain{f_1}$.

We have now shown in Eq.~\eqref{eqn:linears-have-affine-domain} that $\dom
f_1$ is the intersection of an affine set with $\R^k_+$, so if we can show
that $\dom f_1$ is not pierceable (Def.~\ref{def:pierceable}),
Lemma~\ref{lemma:pierceable} will imply that
$\dom f_1 = \{x \in \R^k_+ \mid x_j = 0 ~ \mbox{for} ~ j \in I\}$
for some index set $I$. Indeed, assume
that $x, y \in \R^k_+ \setminus \dom f_1$ satisfy
$z = \half(x + y) \in \dom f_1$, so that $\dom f_1$ is pierceable;
we will show that this implies that $\Omega_1$ is pierceable.
Let $\wt{z} \in \Omega_1$, which is assumed non-empty.
As $\dom f_1$ is closed, for small enough $\epsilon > 0$
we have
\begin{equation*}
  x + \epsilon (\wt{z} - x)
  \not \in \dom f_1
  ~~ \mbox{and} ~~
  y + \epsilon(\wt{z} - y) \not \in \dom f_1.
\end{equation*}
Define $x' = \epsilon \wt{z} + (1 - \epsilon) x$,
$y' = \epsilon \wt{z} + (1 - \epsilon) y$, and $z' = \epsilon \wt{z}
+ (1 - \epsilon) z$, so that
$\half(x' + y') = z'$, where $z' \in \dom f_1$, but by construction
$z' \not \in H$. That is, $z' \in \Omega_1$, and $\Omega_1$ is
pierceable. Now, $z' \not \in \dom f_2$, so the
convexity of $f_2$ implies
\begin{equation*}
  f_2(x') + f_2(y') \ge 2 f_2(z') = \infty,
\end{equation*}
while we know that $x', y' \not \in \dom f_1$ so that $f_1(x') + f_1(y') =
\infty > 2 f_1(z')$, as $z' \in \Omega_1$.  But this contradicts the order
equivalence of $f_1$ and $f_2$, so our assumption that $\dom f_1$ is
pierceable must be false.  Lemma~\ref{lemma:pierceable}, coupled with
Eq.~\eqref{eqn:linears-have-affine-domain}, then implies that
$\dom f_1$ has the form claimed in the statement of the lemma.

If $\Omega_2 = \dom f_2 \setminus H \neq \varnothing$, we may achieve a
similar result by completely paralleling the proof for the set $\Omega_1$
beginning from expression~\eqref{eqn:linears-have-affine-domain},
as the proof uses only convexity of $\dom f_1$ and
that $\dom f_1$ is closed. On the other hand, if
$\Omega_2 = \varnothing$, then we must have
\begin{equation*}
  \domain{f_2} = \domain{f_2} \cap H
  = \domain{f_1} \cap
  \affine{\domain{f_2}} = \domain{f_1} \cap H
  = L \subset \domain{f_1}.
\end{equation*}
Note that $L$ is an affine space intersected with the positive orthant, that
is, $L = \affine{L} \cap \R^k_+$ and that $\domain{f_1} = \{x\in \R_+^k \mid
x_j = 0 ~ \mbox{for} ~j\in I_1\}$ for an index set $I_1$.  Thus
all we need to
show is that $L$ is not pierceable, then apply Lemma~\ref{lemma:pierceable}.
Choose any $x, y \in \R^k_+$ such that $\half(x + y) = z$ for
some $z \in \dom f_2$. Without loss of generality, we may assume
that $x, y \in \dom f_1$ as $z_j = 0$ for all $j \in I_1$, because
$\dom f_2 \subset \dom f_1$. Because $f_1$ is linear on its domain,
we have $f_1(x) + f_1(y) = 2 f_1(z)$, and order equivalence
implies that $f_2(x) + f_2(y) = 2 f_2(z)$. Thus we have
$f_2(x) < \infty$ and $f_2(y) < \infty$, as $z \in \dom f_2$, so
that $L$ is not pierceable. Lemma~\ref{lemma:pierceable} then
implies that
$L = \domain{f_2} = \{x\in \R_+^k \mid x_j = 0 ~ \mbox{for}~ j\in
I_2\}$ for some index set $I_2 \supset I_1$.


\subsection{Proof of Lemma~\ref{lemma:nonempty-intersection}}
\label{sec:proof-nonempty-intersection}

As in the proof of Lemma~\ref{lemma:characterization-linear} (see
Sec.~\ref{sec:proof-characterization-linear}), we know that $\dom f_1$ and
$\dom f_2$ are closed convex sets.

Suppose for the sake of contradiction that $\domain{f_1} \cap \domain{f_2} =
\varnothing$.
Let $H_1 = (\affine{\domain{f_1}}) \cap
\R_+^k$ and $H_2 = (\affine{\domain{f_2}}) \cap \R_+^k$; we
will show that  $\domain{f_1} = H_1$. 
%
Indeed, choose $x \in H_1$ and $y \in \relint \dom f_1$. Then
there exists $\lambda \in (0, 1)$ such that
\begin{equation}
  \label{eqn:pick-a-z-any-z}
  z = \lambda y + (1 - \lambda) x \in \dom f_1
\end{equation}
by standard results in convex analysis
(cf.\ Lemma~\ref{lemma:interior-line-segments}).  Moreover, defining
$z_\epsilon = (1 + \epsilon) z - \epsilon x = z + \epsilon(z - x)$, we
have that $z_\epsilon \not \in \dom f_2$ for small enough $\epsilon > 0$,
as $\dom f_2$ is closed and $z \in \dom f_1$.
Now, consider $z_{-\epsilon} = (1 - \epsilon) z + \epsilon x$, which
also satisfies $z_{-\epsilon} \not \in \dom f_2$ for small $\epsilon > 0$.
We have
\begin{equation*}
  \infty = f_2(z_{-\epsilon}) + f_2(z_\epsilon) = 2 f_2(z),
\end{equation*}
and order equivalence then implies that $f_1(z_{-\epsilon}) +
f_1(z_\epsilon) = 2 f_1(z)$. In particular, $f_1(z_{-\epsilon}) < \infty$
and $f_1(z_\epsilon) < \infty$. Now, if $H_1 \neq \dom f_1$, we could have
chosen $x \in H_1$ with $x \not \in \dom f_1$ and $\lambda \in (0, 1)$
such that $z \in \relbd \dom f_1$ in
expression~\eqref{eqn:pick-a-z-any-z}. In turn, this would imply that for
all $\epsilon > 0$, the point $z_{-\epsilon} = (1 - \epsilon) z + \epsilon
x \not \in \dom f_1$, which is a contradiction. Thus $H_1 = \dom f_1$, and
similarly, $H_2 = \dom f_2$.

We now show that both $\domain{f_1}$ and $\domain{f_2}$ are not
pierceable. For the sake of contradiction assume that $\domain{f_1}$ is
pierceable, so there exist $x, y \not \in \dom f_1$ and $z \in
\domain{f_1}$ such that $\half(x + y) = z$.  Now, since $z \in
(\domain{f_2})^c$ and $(\domain{f_2})^c$ is open set, for sufficiently
small $\epsilon > 0$ we have $x_{\epsilon} \defeq \epsilon x +
(1-\epsilon) z \not\in \domain{f_2}$ and $y_{\epsilon} \defeq \epsilon y +
(1-\epsilon) z \not\in \domain{f_2}$. Therefore, since we have
$f_2(x_{\epsilon}) + f_2(y_{\epsilon}) = +\infty = 2 f_2 (z)$, by order
equivalence, we have $f_1(x_{\epsilon}) + f_1(y_{\epsilon}) = 2 f_1 (z)$.
But this is our desired contradiction, as $f_1(x_{\epsilon}) +
f_1(y_{\epsilon}) = +\infty$ while $ f_1 (z) < +\infty$ because
$z \in \dom f_1$. So $\dom f_1$ is not pierceable, and $\dom f_2$
is similarly not pierceable.

Both $\domain{f_1}$ and $\domain{f_2}$ are affine sets intersected with
$\R_+^k$ that are non-pierceable; using
Lemma~\ref{lemma:pierceable}, both contain 0, and we must have $\dom f_1
\cap \dom f_2 \neq \varnothing$.





%% \begin{lemma}
%%   \label{lemma:existence of ri}
%%   Let $C$ be a nonempty convex set. Then $\relint C$ is nonempty. 
%% \end{lemma}
  
%% \subsection{Proof of Lemma~\ref{lemma:points-in-simplices}}
%% \label{sec:proof-points-in-simplices}



%% \begin{lemma}\label{lemma:linear2}
%%   Let $\Omega \subset \R^k$ be convex with non-empty interior and
%%   $f: \Omega \to \R$ be a closed convex function such that for all
%%   collections of points $x_0, x_1, \ldots x_k$ affinely independent
%%   (Def.~\ref{def:affine-independent}) and $E = \conv\{x_0, \ldots,
%%   x_k\}$, there exist $b_E \in \R^k, c_E \in \R$ such that $f(t) = b_E^T t +
%%   c_E$ for $t \in E$. Then there exist $b \in \R^k, c \in \R$ such
%%   that $f(t) = b^T t + c$ for $t \in \Omega$.
%% \end{lemma}
%% \begin{proof}
%%   We show that for any two points $x, y \in \interior \Omega$ that $\nabla
%%   f(x)$ and $\nabla f(y)$ exist and $\nabla f(x) = \nabla f(y)$.  By
%%   Lemma~\ref{lemma:points-in-simplices}, there exist $x_0, x_1, \ldots, x_k
%%   \in \Omega$ such that $x, y \in \interior E$ for $E = \conv\{x_0, \ldots,
%%   x_k\}$, and 
%%   $f$ is affine on $E$ by assumption.
%%   Consequently, $f$ is differentiable on $\interior E$ with $\nabla f(z)$
%%   constant on $\interior E$, whence $\nabla f(x) = \nabla f(y)$.

%%   Now, we have shown that $\nabla f(z)$ exists on $\interior \Omega$
%%   and is constant, so that $f$ is affine on $\interior \Omega$.
%%   Choose $b \in \R^k$ and $c \in \R$ such that
%%   $f(t) = b^T t + c$ on $\interior \Omega$. Then by
%%   Lemma~\ref{lemma:equal-functions} we have that
%%   $f(t) = b^T t + c$ for all of $\Omega$, as $f$ is closed by assumption
%%   and $t \mapsto b^T t + c$ is continuous.
%% \end{proof}


